Communications in cellular automata

The goal of this paper is to show why the framework of communication complexity seems suitable for the study of cellular automata. Researchers have tackled different algorithmic problems ranging from the complexity of predicting to the decidability of different dynamical properties of cellular automata. But the difference here is that we look for communication protocols arising in the dynamics itself. Our work is guided by the following idea: if we are able to give a protocol describing a cellular automaton, then we can understand its behavior.

==> eptcsdata.tex <==
\providecommand{\eid}{8}


==> rules.tex <==
\subsubsection{Rule 110}
\label{rule110}
We wrote in section \ref{pcompleteness_cc} that the P-completeness of
a rule does not imply much on its communication complexity. In fact,
we now show that rule 110, shown P-complete by D. Woods and T. Neary
in \cite{woodsneary06}, can not be in our polynomial class.
(?????????)


\begin{proposition}
The communication complexity of rule 110 is not in $O(\log n)$.


\begin{proof}

\end{proof}
\end{proposition}

\subsubsection{Rule 30}
\begin{proposition}
  There is no one-round protocol for Rule 30 with
  $X=\{0,1\}^{n-\lfloor n/4\rfloor}$ and $Y=\{0,1\}^{n+1+\lfloor
    n/4\rfloor}$ taking less than $n-\lfloor n/4\rfloor$ bits to
  complete.


\begin{proof}

\end{proof}
\end{proposition}
\label{rule30}

